LTL to B\"uchi Automata Translation: Fast and More Deterministic

We introduce improvements in the algorithm by Gastin and Oddoux translating LTL formulae into B\"uchi automata via very weak alternating co-B\"uchi automata and generalized B\"uchi automata. Several improvements are based on specific properties of any formula where each branch of its syntax tree contains at least one eventually operator and at least one always operator. These changes usually result in faster translations and smaller automata. Other improvements reduce non-determinism in the produced automata. In fact, we modified all the steps of the original algorithm and its implementation known as LTL2BA. Experimental results show that our modifications are real improvements. Their implementations within an LTL2BA translation made LTL2BA very competitive with the current version of SPOT, sometimes outperforming it substantially.

==> tabs/big_2-fair_3-2.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\ \hline \hline
  LTL2BA
& 1\,898 & 9\,550 & 1.53 & 2 \\
\hline
%  LTL3BA
%& 1\,738 & 10\'117 & 1.25 & 2 \\
%\hline
  LTL3BA
& 1\,738 & 12\,495 & 0.84 & 23 \\
\hline
  SPOT
%& 1\,412 & 8\,466 & 5.29 & 2 \\
%\hline
%  SPOT, +det
& 1\'412 & 8\,466 & 5.63 & 22 \\
\hline
  SPOT + WDBA min
& 1\,412 & 8\,466 & 3772.27 & 22 \\
\hline
\end{tabular}


==> tabs/big_2.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\ \hline \hline
  LTL2BA
& 2\,118 & 9\,000 & 0.76 s & 25 \\
\hline
%  LTL3BA
%& 1\,551 & 5\,436 & 1.24 s & 32 \\
%\hline
  LTL3BA
& 1\,544 & 5\,535 & 1.15 s & 59 \\
\hline
  SPOT
%& 1\,561 & 5\,729 & 7.88 & 42 \\
%\hline
%  SPOT, +det
& 1\,561 & 5\,729 & 7.93 s & 55 \\
\hline
  SPOT + WDBA min
& 1\,587 & 5\,880 & 11.41 s & 88 \\
\hline
\end{tabular}


==> tabs/big_3.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\ \hline \hline
  LTL2BA
& 24\,648 & 232\,400 & 18.77 & 84 \\
\hline
%  LTL3BA
%& 14\,460 & 92\,080 & 13.50 & 104 \\
%\hline
  LTL3BA
& 13\,990 & 89\,007 & 7.86 & 246 \\
\hline
  SPOT
%& 14\,687 & 95\,616 & 68.05 & 138 \\
%\hline
%  SPOT, +det
& 14\,697 & 95\,645 & 70.08 & 221 \\
\hline
  SPOT + WDBA min\footnotemark[\value{footnote}]
  %{Note that ``SPOT + WDBA min'' failed to translate 6 formula in the one hour limit. Therefore, we the results in braces.}
%& 13\,097 (14\,408) & 77\,346 (94\,248) & 5\,767.92 (5\,770.9) & 373 \\
& 13\,097 & 77\,346 & 5\,767.92 & 373 \\
& (14\,408) & (94\,248) & (5\,770.9) & (373) \\
\hline
\end{tabular}


==> tabs/cichon-alpha.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba} 
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1	&	4	&	9	&	0.104	&	4	&	9	&	0.034	&	4	&	9	&	0.045 \\
\hline
2	&	9	&	36	&	0.093	&	12	&	55	&	0.034	&	9	&	36	&	0.047 \\
\hline
3	&	16	&	100	&	0.096	&	25	&	176	&	0.033	&	16	&	100	&	0.044 \\
\hline
4	&	25	&	225	&	0.109	&	44	&	439	&	0.034	&	25	&	225	&	0.042 \\
\hline
5	&	36	&	441	&	0.126	&	69	&	925	&	0.041	&	36	&	441	&	0.047 \\
\hline
6	&	49	&	784	&	0.170	&	100	&	1733	&	0.044	&	49	&	784	&	0.049 \\
\hline
7	&	64	&	1296	&	0.260	&	137	&	2980	&	0.059	&	64	&	1296	&	0.051 \\
\hline
8	&	81	&	2025	&	0.413	&	180	&	4801	&	0.084	&	81	&	2025	&	0.067 \\
\hline
9	&	100	&	3025	&	0.659	&	229	&	7349	&	0.120	&	100	&	3025	&	0.078 \\
\hline
10	&	121	&	4356	&	1.035	&	284	&	10795	&	0.167	&	121	&	4356	&	0.093 \\
\hline
11	&	144	&	6084	&	1.628	&	345	&	15328	&	0.286	&	144	&	6084	&	0.126 \\
\hline
12	&	169	&	8281	&	2.471	&	412	&	21155	&	0.472	&	169	&	8281	&	0.170 \\
\hline
13	&	196	&	11025	&	3.730	&	485	&	28501	&	0.731	&	196	&	11025	&	0.222 \\
\hline
14	&	225	&	14400	&	5.479	&	564	&	37609	&	1.139	&	225	&	14400	&	0.287 \\
\hline
15	&	256	&	18496	&	7.914	&	649	&	48740	&	1.719	&	256	&	18496	&	0.367 \\
\hline
16	&	289	&	23409	&	11.291	&	740	&	62173	&	2.625	&	289	&	23409	&	0.532 \\
\hline
17	&	324	&	29241	&	15.517	&	837	&	78205	&	3.826	&	324	&	29241	&	0.700 \\
\hline
18	&	361	&	36100	&	21.336	&	940	&	97151	&	6.683	&	361	&	36100	&	0.903 \\
\hline
19	&	400	&	44100	&	28.436	&	1049	&	119344	&	7.785	&	400	&	44100	&	1.136 \\
\hline
20	&	441	&	53361	&	37.832	&	1164	&	145135	&	10.969	&	441	&	53361	&	1.456 \\
\hline
\end{tabular}


==> tabs/cichon-beta.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba} 
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 &	4	&	10	&	0.083	&	4	&	9	&	0.053	&	4	&	9	&	0.063 \\
\hline
2 &	9	&	16	&	0.079	&	9	&	16	&	0.032	&	9	&	16	&	0.056 \\
\hline
3 &	16	&	25	&	0.072	&	16	&	25	&	0.032	&	16	&	25	&	0.054 \\
\hline
4 &	25	&	36	&	0.068	&	25	&	36	&	0.033	&	25	&	36	&	0.056 \\
\hline
5 &	36	&	49	&	0.060	&	36	&	49	&	0.038	&	36	&	49	&	0.050 \\
\hline
6 &	49	&	64	&	0.068	&	49	&	64	&	0.035	&	49	&	64	&	0.058 \\
\hline
7 &	64	&	81	&	0.069	&	64	&	81	&	0.034	&	64	&	81	&	0.048 \\
\hline
8 &	81	&	100	&	0.080	&	81	&	100	&	0.035	&	81	&	100	&	0.054 \\
\hline
9 &	100	&	121	&	0.092	&	100	&	121	&	0.037	&	100	&	121	&	0.057 \\
\hline
10 &	121	&	144	&	0.092	&	121	&	144	&	0.039	&	121	&	144	&	0.057 \\
\hline
11 &	144	&	169	&	0.099	&	144	&	169	&	0.043	&	144	&	169	&	0.058 \\
\hline
12 &	169	&	196	&	0.101	&	169	&	196	&	0.045	&	169	&	196	&	0.063 \\
\hline
13 &	196	&	225	&	0.094	&	196	&	225	&	0.051	&	196	&	225	&	0.059 \\
\hline
14 &	225	&	256	&	0.097	&	225	&	256	&	0.052	&	225	&	256	&	0.058 \\
\hline
15 &	256	&	289	&	0.088	&	256	&	289	&	0.050	&	256	&	289	&	0.067 \\
\hline
16 &	289	&	324	&	0.099	&	289	&	324	&	0.052	&	289	&	324	&	0.062 \\
\hline
17 &	324	&	361	&	0.101	&	324	&	361	&	0.054	&	324	&	361	&	0.064 \\
\hline
18 &	361	&	400	&	0.112	&	361	&	400	&	0.045	&	361	&	400	&	0.071 \\
\hline
19 &	400	&	441	&	0.110	&	400	&	441	&	0.054	&	400	&	441	&	0.071 \\
\hline
20 &	441	&	484	&	0.114	&	441	&	484	&	0.064	&	441	&	484	&	0.073 \\
\hline
\end{tabular}


==> tabs/cichon-beta2.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba} 
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1	&	4	&	10	&	0.085	&	4	&	9	&	0.044	&	4	&	9	&	0.041 \\
\hline
2	&	9	&	16	&	0.096	&	9	&	16	&	0.043	&	9	&	16	&	0.049 \\
\hline
3	&	16	&	25	&	0.116	&	16	&	25	&	0.068	&	16	&	25	&	0.065 \\
\hline
4	&	25	&	36	&	0.124	&	25	&	36	&	0.080	&	25	&	36	&	0.076 \\
\hline
5	&	36	&	49	&	0.128	&	36	&	49	&	0.089	&	36	&	49	&	0.096 \\
\hline
6	&	49	&	64	&	0.155	&	49	&	64	&	0.112	&	49	&	64	&	0.116 \\
\hline
7	&	64	&	81	&	0.165	&	64	&	81	&	0.134	&	64	&	81	&	0.127 \\
\hline
8	&	81	&	100	&	0.171	&	81	&	100	&	0.161	&	81	&	100	&	0.146 \\
\hline
9	&	100	&	121	&	0.185	&	100	&	121	&	0.196	&	100	&	121	&	0.165 \\
\hline
10	&	121	&	144	&	0.194	&	121	&	144	&	0.304	&	121	&	144	&	0.177 \\
\hline
11	&	144	&	169	&	0.247	&	144	&	169	&	0.633	&	144	&	169	&	0.198 \\
\hline
12	&	169	&	196	&	0.242	&	169	&	196	&	1.928	&	169	&	196	&	0.212 \\
\hline
13	&	196	&	225	&	0.229	&	196	&	225	&	7.095	&	196	&	225	&	0.232 \\
\hline
14	&	225	&	256	&	0.272	&	225	&	256	&	28.341	&	225	&	256	&	0.242 \\
\hline
15	&	256	&	289	&	0.309	&	256	&	289	&	1m51.655	&	256	&	289	&	0.256 \\
\hline
16	&	289	&	324	&	0.333	&	289	&	324	&	7m32.909	&	289	&	324	&	0.279 \\
\hline
17	&	324	&	361	&	0.309	&	324	&	361	&	30m47.817	&	324	&	361	&	0.284 \\
\hline
18	&	361	&	400	&	0.419	&	--	&	--	&	--	&	361	&	400	&	0.325 \\
\hline
19	&	400	&	441	&	0.384	&	--	&	--	&	--	&	400	&	441	&	0.323 \\
\hline
20	&	441	&	484	&	0.381	&	--	&	--	&	--	&	441	&	484	&	0.353 \\
\hline
\end{tabular}


==> tabs/cichon-psi.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba} 
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1	&	2	&	4	&	0.087	&	2	&	4	&	0.027	&	2	&	4	&	0.050 \\
\hline
2	&	3	&	8	&	0.074	&	3	&	8	&	0.025	&	3	&	8	&	0.046 \\
\hline
3	&	4	&	13	&	0.077	&	4	&	13	&	0.025	&	4	&	13	&	0.047 \\
\hline
4	&	5	&	19	&	0.079	&	5	&	19	&	0.025	&	5	&	19	&	0.048 \\
\hline
5	&	6	&	26	&	0.068	&	6	&	26	&	0.039	&	6	&	26	&	0.046 \\
\hline
6	&	7	&	34	&	0.071	&	7	&	34	&	0.083	&	7	&	34	&	0.049 \\
\hline
7	&	8	&	43	&	0.077	&	8	&	43	&	0.441	&	8	&	43	&	0.044 \\
\hline
8	&	9	&	53	&	0.092	&	9	&	53	&	4.730	&	9	&	53	&	0.045 \\
\hline
9	&	10	&	64	&	0.101	&	10	&	64	&	43.380	&	10	&	64	&	0.050 \\
\hline
10	&	11	&	76	&	0.142	&	11	&	76	&	8m57.889	&	11	&	76	&	0.060 \\
\hline
11	&	12	&	89	&	0.225	&	--	&	--	&	--	&	12	&	89	&	0.074 \\
\hline
12	&	13	&	103	&	0.418	&	--	&	--	&	--	&	13	&	103	&	0.110 \\
\hline
13	&	14	&	118	&	0.932	&	--	&	--	&	--	&	14	&	118	&	0.193 \\
\hline
14	&	15	&	134	&	1.961	&	--	&	--	&	--	&	15	&	134	&	0.366 \\
\hline
15	&	16	&	151	&	4.632	&	--	&	--	&	--	&	16	&	151	&	0.752 \\
\hline
16	&	17	&	169	&	9.792	&	--	&	--	&	--	&	17	&	169	&	1.772 \\
\hline
17	&	18	&	188	&	24.274	&	--	&	--	&	--	&	18	&	188	&	3.795 \\
\hline
18	&	19	&	208	&	1m1.941	&	--	&	--	&	--	&	19	&	208	&	8.725 \\
\hline
19	&	20	&	229	&	3m9.427	&	--	&	--	&	--	&	20	&	229	&	20.337 \\
\hline
20	&	21	&	251	&	9m39.981	&	--	&	--	&	--	&	21	&	251	&	53.471 \\
\hline
\end{tabular}


==> tabs/cichon-xi.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba} 
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1	&	2	&	3	&	0.082	&	2	&	3	&	0.026	&	2	&	3	&	0.051 \\
\hline
2	&	3	&	5	&	0.077	&	3	&	5	&	0.023	&	3	&	5	&	0.049 \\
\hline
3	&	4	&	7	&	0.072	&	4	&	7	&	0.022	&	4	&	7	&	0.048 \\
\hline
4	&	5	&	9	&	0.074	&	5	&	9	&	0.038	&	5	&	9	&	0.042 \\
\hline
5	&	6	&	11	&	0.078	&	6	&	11	&	0.023	&	6	&	11	&	0.050 \\
\hline
6	&	7	&	13	&	0.076	&	7	&	13	&	0.023	&	7	&	13	&	0.045 \\
\hline
7	&	8	&	15	&	0.081	&	8	&	15	&	0.024	&	8	&	15	&	0.047 \\
\hline
8	&	9	&	17	&	0.077	&	9	&	17	&	0.026	&	9	&	17	&	0.037 \\
\hline
9	&	10	&	19	&	0.080	&	10	&	19	&	0.025	&	10	&	19	&	0.037 \\
\hline
10	&	11	&	21	&	0.081	&	11	&	21	&	0.026	&	11	&	21	&	0.050 \\
\hline
11	&	12	&	23	&	0.082	&	12	&	23	&	0.023	&	12	&	23	&	0.042 \\
\hline
12	&	13	&	25	&	0.082	&	13	&	25	&	0.023	&	13	&	25	&	0.045 \\
\hline
13	&	14	&	27	&	0.076	&	14	&	27	&	0.024	&	14	&	27	&	0.042 \\
\hline
14	&	15	&	29	&	0.079	&	15	&	29	&	0.024	&	15	&	29	&	0.049 \\
\hline
15	&	16	&	31	&	0.088	&	16	&	31	&	0.024	&	16	&	31	&	0.040 \\
\hline
16	&	17	&	33	&	0.077	&	17	&	33	&	0.024	&	17	&	33	&	0.046 \\
\hline
17	&	18	&	35	&	0.081	&	18	&	35	&	0.025	&	18	&	35	&	0.043 \\
\hline
18	&	19	&	37	&	0.082	&	19	&	37	&	0.023	&	19	&	37	&	0.054 \\
\hline
19	&	20	&	39	&	0.060	&	20	&	39	&	0.024	&	20	&	39	&	0.051 \\
\hline
20	&	21	&	41	&	0.079	&	21	&	41	&	0.024	&	21	&	41	&	0.047 \\
\hline
\end{tabular}


==> tabs/impr-big_2-fair_1.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\
\hline \hline
  SPOT
& 2\,400 & 12\,608 & 5.89 & 2 \\
\hline
  SPOT + WDBA min
& 2\,400 & 12\,608 & 483.88 & 2 \\
\hline
  LTL2BA
& 3\,493 & 19\,762 & 0.83 & 2 \\
\hline
  LTL3BA + form. red.
& 2\,744 & 14\,207 & 0.78 & 2 \\
\hline
  LTL3BA + form. red., VWAA
& 2\,744 & 15\,645 & 0.81 & 2 \\
\hline
  LTL3BA + form. red., VWAA, TGBA
& 2\,399 & 11\,686 & 0.80 & 2 \\
\hline
  LTL3BA + form. red., VWAA, TGBA, BA
& 2\,288 & 11\,142 & 0.83 & 2 \\
\hline
\end{tabular}


==> tabs/impr-big_2-fair_3-2.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\
\hline \hline
  SPOT
& 1\,412 & 8\,466 & 5.53 & 22 \\
\hline
  SPOT + WDBA min
& 1\,412 & 8\,466 & 3\,784.37 & 22 \\
\hline
  LTL2BA
& 1\,898 & 9\,550 & 1.47 & 2 \\
\hline
  LTL3BA + form. red.
& 1\,567 & 7\,477 & 1.05 & 2 \\
\hline
  LTL3BA + form. red., VWAA
& 1\,698 & 12\,288 & 0.92 & 22 \\
\hline
  LTL3BA + form. red., VWAA, TGBA
& 1\,732 & 12\,479 & 0.90 & 22 \\
\hline
  LTL3BA + form. red., VWAA, TGBA, BA
& 1\,659 & 11\,979 & 0.85 & 22 \\
\hline
\end{tabular}


==> tabs/impr-big_2.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\
\hline \hline
  SPOT
& 1\,561 & 5\,729 & 7.47 & 55 \\
\hline
  SPOT + WDBA min
& 1\,587 & 5\,880 & 10.81 & 88 \\
\hline
  LTL2BA
& 2\,118 & 9\,000 & 0.81 & 25 \\
\hline
  LTL3BA + form. red.
& 1\,621 & 5\,865 & 1.26 & 27 \\
\hline
  LTL3BA + form. red., VWAA
& 1\,631 & 6\,094 & 1.41 & 54 \\
\hline
  LTL3BA + form. red., VWAA, TGBA
& 1\,565 & 5\,615 & 1.41 & 54 \\
\hline
  LTL3BA + form. red., VWAA, TGBA, BA
& 1\,507 & 5\,348 & 1.38 & 54 \\
\hline
\end{tabular}


==> tabs/impr-big_3.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\
\hline \hline
  SPOT
& 14\,697 & 95\,645 & 68.46 & 221 \\
\hline
  SPOT + WDBA min
& 13\,097 & 77\,346 & 5\,916.45 & 373 \\
& (14\,408) & (94\,248) & (5\,919.43) & (373) \\
\hline
  LTL2BA
& 24\,648 & 232\,400 & 18.57 & 84 \\
\hline
  LTL3BA + form. red.
& 17\,107 & 129\,774 & 22.25 & 92 \\
\hline
  LTL3BA + form. red., VWAA
& 15\,936 & 115\,624 & 9.04 & 237 \\
\hline
  LTL3BA + form. red., VWAA, TGBA
& 14\,113 & 91\,159 & 8.53 & 240 \\
\hline
  LTL3BA + form. red., VWAA, TGBA, BA
& 13\,244 & 85\,511 & 8.30 & 240 \\
\hline
\end{tabular}


==> tabs/impr-fg.tex <==
\begin{tabular}{|l||c|c|c|c|}
\hline
Translator & States & Transitions & Time & \# of det. \\
\hline \hline
  SPOT
& 1\,230 & 4\,131 & 11.00 & 34 \\
\hline
  SPOT + WDBA min
& 1\,236 & 4\,179 & 21.15 & 38 \\
\hline
  LTL2BA
& 1\,817 & 7\,088 & 0.79 & 13 \\
\hline
  LTL3BA + form. red.
& 1\,621 & 6\,086 & 1.55 & 10 \\
\hline
  LTL3BA + form. red., VWAA
& 1\,597 & 5\,651 & 1.46 & 29 \\
\hline
  LTL3BA + form. red., VWAA, TGBA
& 1\,358 & 4\,098 & 1.52 & 31 \\
\hline
  LTL3BA + form. red., VWAA, TGBA, BA
& 1\,341 & 4\,036 & 1.39 & 31 \\
\hline
\end{tabular}


==> tabs/ltl_c1.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 2 & 4 & 0.055 & 2 & 4 & 0.006 & 2 & 4 & 0.017 \\
\hline
2 & 2 & 4 & 0.057 & 2 & 4 & 0.006 & 2 & 4 & 0.013 \\
\hline
4 & 2 & 4 & 0.058 & 2 & 4 & 0.007 & 2 & 4 & 0.014 \\
\hline
8 & 2 & 4 & 0.060 & 2 & 4 & 0.007 & 2 & 4 & 0.014 \\
\hline
16 & 2 & 4 & 0.064 & 2 & 4 & 0.008 & 2 & 4 & 0.013 \\
\hline
32 & 2 & 4 & 0.068 & 2 & 4 & 0.009 & 2 & 4 & 0.016 \\
\hline
64 & 2 & 4 & 0.081 & 2 & 4 & 0.025 & 2 & 4 & 0.018 \\
\hline
128 & 2 & 4 & 0.093 & 2 & 4 & 0.104 & 2 & 4 & 0.048 \\
\hline
256 & 2 & 4 & 0.165 & 2 & 4 & 0.959 & 2 & 4 & 0.233 \\
\hline
512 & 2 & 4 & 0.465 & & & & 2 & 4 & 1.655 \\
\hline
1024 & 2 & 4 & 1.938 & & & & 2 & 4 & 13.079 \\
\hline
2048 & 2 & 4 & 7.838 & & & & 2 & 4 & 105.678 \\
\hline
4096 & 2 & 4 & 31.681 & & & & 2 & 4 & 900.971 \\
\hline
8192 & 2 & 4 & 129.695 & & & & & & \\
\hline
16384 & 2 & 4 & 510.516 & & & & & & \\
\hline
32768 & 2 & 4 & 2187.611 & & & & & & \\
\hline
\end{tabular}


==> tabs/ltl_c2.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 2 & 4 & 0.109 & 2 & 4 & 0.024 & 2 & 4 & 0.030 \\
\hline
2 & 3 & 8 & 0.085 & 3 & 8 & 0.025 & 3 & 8 & 0.031 \\
\hline
3 & 4 & 13 & 0.089 & 4 & 13 & 0.027 & 4 & 13 & 0.032 \\
\hline
4 & 5 & 19 & 0.082 & 5 & 19 & 0.029 & 5 & 19 & 0.033 \\
\hline
5 & 6 & 26 & 0.087 & 6 & 26 & 0.040 & 6 & 26 & 0.034 \\
\hline
6 & 7 & 34 & 0.080 & 7 & 34 & 0.088 & 7 & 34 & 0.035 \\
\hline
7 & 8 & 43 & 0.086 & 8 & 43 & 0.474 & 8 & 43 & 0.036 \\
\hline
8 & 9 & 53 & 0.089 & 9 & 53 & 4.939 & 9 & 53 & 0.038 \\
\hline
9 & 10 & 64 & 0.115 & 10 & 64 & 42.812 & 10 & 64 & 0.046 \\
\hline
10 & 11 & 76 & 0.148 & 11 & 76 & 550.528 & 11 & 76 & 0.048 \\
\hline
11 & 12 & 89 & 0.240 & & & & 12 & 89 & 0.067 \\
\hline
12 & 13 & 103 & 0.429 & & & & 13 & 103 & 0.109 \\
\hline
13 & 14 & 118 & 0.874 & & & & 14 & 118 & 0.189 \\
\hline
14 & 15 & 134 & 1.943 & & & & 15 & 134 & 0.358 \\
\hline
15 & 16 & 151 & 4.239 & & & & 16 & 151 & 0.726 \\
\hline
16 & 17 & 169 & 9.521 & & & & 17 & 169 & 1.777 \\
\hline
17 & 18 & 188 & 22.861 & & & & 18 & 188 & 3.808 \\
\hline
18 & 19 & 208 & 55.426 & & & & 19 & 208 & 8.987 \\
\hline
19 & 20 & 229 & 149.244 & & & & 20 & 229 & 19.748 \\
\hline
20 & 21 & 251 & 409.208 & & & & 21 & 251 & 44.953 \\
\hline
21 & 22 & 274 & 1036.646 & & & & 22 & 274 & 105.223 \\
\hline
22 & 23 & 298 & 2446.903 & & & & 23 & 298 & 258.433 \\
\hline
23 & & & & & & & 24 & 323 & 749.488 \\
\hline
24 & & & & & & & 25 & 349 & 2488.576 \\
\hline
\end{tabular}


==> tabs/ltl_e.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 2 & 3 & 0.073 & 2 & 3 & 0.022 & 2 & 3 & 0.024 \\
\hline
2 & 4 & 9 & 0.076 & 4 & 9 & 0.023 & 4 & 9 & 0.025 \\
\hline
3 & 8 & 27 & 0.080 & 8 & 27 & 0.023 & 8 & 27 & 0.028 \\
\hline
4 & 16 & 81 & 0.082 & 16 & 81 & 0.023 & 16 & 81 & 0.031 \\
\hline
5 & 32 & 243 & 0.088 & 32 & 243 & 0.024 & 32 & 243 & 0.034 \\
\hline
6 & 64 & 729 & 0.114 & 64 & 729 & 0.029 & 64 & 729 & 0.037 \\
\hline
7 & 128 & 2187 & 0.224 & 128 & 2187 & 0.038 & 128 & 2187 & 0.044 \\
\hline
8 & 256 & 6561 & 0.629 & 256 & 6561 & 0.081 & 256 & 6561 & 0.073 \\
\hline
9 & 512 & 19683 & 2.033 & 512 & 19683 & 0.291 & 512 & 19683 & 0.174 \\
\hline
10 & 1024 & 59049 & 7.018 & 1024 & 59049 & 1.450 & 1024 & 59049 & 0.642 \\
\hline
11 & 2048 & 177147 & 23.727 & 2048 & 177147 & 8.427 & 2048 & 177147 & 2.783 \\
\hline
12 & 4096 & 531441 & 81.912 & 4096 & 531441 & 53.930 & 4096 & 531441 & 12.254 \\
\hline
13 & 8192 & 1594323 & 280.942 & 8192 & 1594323 & 514.879 & 8192 & 1594323 & 55.724 \\
\hline
14 & 16384 & 4782969 & 1025.091 & 16384 & 4782969 & 3357.356 & 16384 & 4782969 & 257.271 \\
\hline
15 & & & & & & & 32768 & 14348907 & 1223.646 \\
\hline
\end{tabular}


==> tabs/ltl_q.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 4 & 7 & 0.082 & 4 & 7 & 0.028 & 4 & 7 & 0.038 \\
\hline
2 & 8 & 20 & 0.082 & 9 & 22 & 0.029 & 9 & 22 & 0.038 \\
\hline
3 & 18 & 60 & 0.095 & 22 & 69 & 0.032 & 22 & 69 & 0.040 \\
\hline
4 & 42 & 183 & 0.098 & 56 & 219 & 0.035 & 56 & 219 & 0.045 \\
\hline
5 & 100 & 568 & 0.115 & 145 & 704 & 0.047 & 145 & 704 & 0.046 \\
\hline
6 & 240 & 1788 & 0.194 & 378 & 2289 & 0.071 & 378 & 2289 & 0.060 \\
\hline
7 & 578 & 5693 & 0.426 & 988 & 7515 & 0.256 & 988 & 7515 & 0.132 \\
\hline
8 & 1394 & 18290 & 1.240 & 2585 & 24872 & 1.609 & 2585 & 24872 & 0.495 \\
\hline
9 & 3364 & 59170 & 3.994 & 6766 & 82861 & 13.074 & 6766 & 82861 & 2.789 \\
\hline
10 & 8120 & 192437 & 13.648 & 17712 & 277519 & 95.680 & 17712 & 277519 & 17.786 \\
\hline
11 & 19602 & 628362 & 46.274 & 46369 & 933408 & 2914.971 & 46369 & 933408 & 114.445 \\
\hline
12 & 47322 & 2057922 & 157.249 & & & & 121394 & 3149937 & 1043.299 \\
\hline
13 & 114244 & 6754807 & 579.835 & & & & & & \\
\hline
14 & 275808 & 22208100 & 2199.954 & & & & & & \\
\hline
\end{tabular}


==> tabs/ltl_r.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 5 & 11 & 0.082 & 5 & 11 & 0.026 & 5 & 11 & 0.033 \\
\hline
2 & 14 & 43 & 0.090 & 13 & 37 & 0.028 & 14 & 40 & 0.039 \\
\hline
3 & 42 & 164 & 0.099 & 36 & 122 & 0.032 & 40 & 136 & 0.044 \\
\hline
4 & 128 & 626 & 0.122 & 102 & 414 & 0.046 & 114 & 461 & 0.048 \\
\hline
5 & 390 & 2406 & 0.214 & 292 & 1454 & 0.100 & 324 & 1592 & 0.058 \\
\hline
6 & 1184 & 9322 & 0.638 & 842 & 5271 & 1.128 & 922 & 5647 & 0.106 \\
\hline
7 & 3582 & 36382 & 2.581 & 2444 & 19618 & 16.362 & 2636 & 20594 & 0.466 \\
\hline
8 & 10808 & 142842 & 11.901 & 7138 & 74521 & 635.161 & 7586 & 76969 & 3.095 \\
\hline
9 & 32550 & 563438 & 54.820 & & & & 21988 & 293356 & 23.177 \\
\hline
10 & 97904 & 2230346 & 252.664 & & & & 64170 & 1134515 & 183.206 \\
\hline
11 & 294222 & 8852190 & 1401.871 & & & & 188412 & 4433414 & 3386.277 \\
\hline
\end{tabular}


==> tabs/ltl_s.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 1 & 1 & 0.060 & 1 & 1 & 0.007 & 1 & 1 & 0.018 \\
\hline
2 & 1 & 1 & 0.061 & 1 & 1 & 0.006 & 1 & 1 & 0.013 \\
\hline
4 & 1 & 1 & 0.063 & 1 & 1 & 0.006 & 1 & 1 & 0.014 \\
\hline
8 & 1 & 1 & 0.065 & 1 & 1 & 0.005 & 1 & 1 & 0.014 \\
\hline
16 & 1 & 1 & 0.067 & 1 & 1 & 0.006 & 1 & 1 & 0.016 \\
\hline
32 & 1 & 1 & 0.069 & 1 & 1 & 0.007 & 1 & 1 & 0.014 \\
\hline
64 & 1 & 1 & 0.071 & 1 & 1 & 0.007 & 1 & 1 & 0.015 \\
\hline
128 & 1 & 1 & 0.083 & 1 & 1 & 0.006 & 1 & 1 & 0.022 \\
\hline
256 & 1 & 1 & 0.151 & 1 & 1 & 0.009 & 1 & 1 & 0.042 \\
\hline
512 & 1 & 1 & 0.426 & & & & 1 & 1 & 0.113 \\
\hline
1024 & 1 & 1 & 1.511 & & & & 1 & 1 & 0.545 \\
\hline
2048 & 1 & 1 & 6.608 & & & & 1 & 1 & 5.148 \\
\hline
4096 & 1 & 1 & 25.851 & & & & 1 & 1 & 83.036 \\
\hline
8192 & 1 & 1 & 106.276 & & & & 1 & 1 & 1336.912 \\
\hline
16384 & 1 & 1 & 430.801 & & & & & & \\
\hline
32768 & 1 & 1 & 1772.321 & & & & & & \\
\hline
\end{tabular}


==> tabs/ltl_u1.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 2 & 2 & 0.078 & 2 & 2 & 0.024 & 2 & 2 & 0.033 \\
\hline
2 & 2 & 3 & 0.080 & 2 & 3 & 0.025 & 2 & 3 & 0.034 \\
\hline
3 & 4 & 10 & 0.083 & 6 & 17 & 0.025 & 6 & 17 & 0.035 \\
\hline
4 & 8 & 34 & 0.086 & 15 & 73 & 0.026 & 15 & 73 & 0.037 \\
\hline
5 & 16 & 116 & 0.089 & 37 & 311 & 0.030 & 37 & 311 & 0.039 \\
\hline
6 & 32 & 396 & 0.104 & 89 & 1290 & 0.037 & 89 & 1290 & 0.045 \\
\hline
7 & 64 & 1352 & 0.166 & 209 & 5207 & 0.074 & 209 & 5207 & 0.093 \\
\hline
8 & 128 & 4616 & 0.458 & 481 & 20548 & 0.432 & 481 & 20548 & 0.569 \\
\hline
9 & 256 & 15760 & 1.582 & 1089 & 79649 & 5.117 & 1089 & 79649 & 7.529 \\
\hline
10 & 512 & 53808 & 6.103 & 2433 & 304394 & 83.984 & 2433 & 304394 & 132.600 \\
\hline
11 & 1024 & 183712 & 24.535 & 5377 & 1150123 & 1799.934 & 5377 & 1150123 & 2876.111 \\
\hline
12 & 2048 & 627232 & 95.885 & & & & & & \\
\hline
13 & 4096 & 2141504 & 386.997 & & & & & & \\
\hline
14 & 8192 & 7311552 & 1501.769 & & & & & & \\
\hline
\end{tabular}


==> tabs/ltl_u2.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 2 & 2 & 0.024 & 2 & 2 & 0.006 & 2 & 2 & 0.021 \\
\hline
2 & 2 & 3 & 0.025 & 2 & 3 & 0.005 & 2 & 3 & 0.013 \\
\hline
3 & 6 & 17 & 0.025 & 4 & 10 & 0.006 & 4 & 10 & 0.015 \\
\hline
4 & 15 & 73 & 0.026 & 8 & 36 & 0.006 & 8 & 36 & 0.016 \\
\hline
5 & 37 & 311 & 0.030 & 16 & 136 & 0.010 & 16 & 136 & 0.019 \\
\hline
6 & 89 & 1290 & 0.037 & 32 & 528 & 0.031 & 32 & 528 & 0.032 \\
\hline
7 & 209 & 5207 & 0.074 & 64 & 2080 & 0.301 & 64 & 2080 & 0.164 \\
\hline
8 & 481 & 20548 & 0.432 & 128 & 8256 & 5.350 & 128 & 8256 & 1.697 \\
\hline
9 & 1089 & 79649 & 5.117 & 256 & 32896 & 123.168 & 256 & 32896 & 21.878 \\
\hline
10 & 2433 & 304394 & 83.984 & & & & 512 & 131328 & 324.169 \\
\hline
11 & 5377 & 1150123 & 1799.934 & & & & & & \\
\hline
\end{tabular}


==> tabs/theta.tex <==
\begin{tabular}{|c||*{2}{c|c|c||}c|c|c|}
\hline
& \multicolumn{3}{c||}{Spot} & \multicolumn{3}{c||}{ltl2ba}
& \multicolumn{3}{c|}{ltl3ba} \\
\cline{2-4} \cline{5-7} \cline{8-10}
& St. & Tr. & Time & St. & Tr. & Time & St. & Tr. & Time \\
\hline
\hline
1 & 3 & 7 & 0.083 & 3 & 6 & 0.020 & 3 & 6 & 0.028 \\
\hline
2 & 6 & 20 & 0.081 & 4 & 10 & 0.021 & 4 & 10 & 0.029 \\
\hline
3 & 8 & 33 & 0.087 & 5 & 15 & 0.028 & 5 & 15 & 0.030 \\
\hline
4 & 10 & 49 & 0.083 & 6 & 21 & 0.033 & 6 & 21 & 0.032 \\
\hline
5 & 12 & 68 & 0.091 & 7 & 28 & 0.050 & 7 & 28 & 0.033 \\
\hline
6 & 14 & 90 & 0.097 & 8 & 36 & 0.243 & 8 & 36 & 0.036 \\
\hline
7 & 16 & 115 & 0.106 & 9 & 45 & 1.727 & 9 & 45 & 0.038 \\
\hline
8 & 18 & 143 & 0.121 & 10 & 55 & 18.760 & 10 & 55 & 0.043 \\
\hline
9 & 20 & 174 & 0.184 & 11 & 66 & 175.794 & 11 & 66 & 0.045 \\
\hline
10 & 22 & 208 & 0.314 & 12 & 78 & 2796.799 & 12 & 78 & 0.056 \\
\hline
11 & 24 & 245 & 0.642 & & & & 13 & 91 & 0.085 \\
\hline
12 & 26 & 285 & 1.366 & & & & 14 & 105 & 0.128 \\
\hline
13 & 28 & 328 & 3.198 & & & & 15 & 120 & 0.245 \\
\hline
14 & 30 & 374 & 7.056 & & & & 16 & 136 & 0.519 \\
\hline
15 & 32 & 423 & 16.750 & & & & 17 & 153 & 1.080 \\
\hline
16 & 34 & 475 & 37.959 & & & & 18 & 171 & 2.268 \\
\hline
17 & 36 & 530 & 104.032 & & & & 19 & 190 & 5.009 \\
\hline
18 & 38 & 588 & 295.395 & & & & 20 & 210 & 12.352 \\
\hline
19 & 40 & 649 & 1138.159 & & & & 21 & 231 & 29.419 \\
\hline
20 & 42 & 713 & 1716.512 & & & & 22 & 253 & 72.378 \\
\hline
21 & & & & & & & 23 & 276 & 188.229 \\
\hline
22 & & & & & & & 24 & 300 & 541.048 \\
\hline
23 & & & & & & & 25 & 325 & 1637.417 \\
\hline
\end{tabular}

